KV-match: A Subsequence Matching Approach Supporting Normalization and Time Warping [Extended Version]

The volume of time series data has exploded due to the popularity of new applications, such as data center management and IoT. Subsequence matching is a fundamental task in mining time series data. All index-based approaches only consider raw subsequence matching (RSM) and do not support subsequence normalization. UCR Suite can deal with normalized subsequence match problem (NSM), but it needs to scan full time series. In this paper, we propose a novel problem, named constrained normalized subsequence matching problem (cNSM), which adds some constraints to NSM problem. The cNSM problem provides a knob to flexibly control the degree of offset shifting and amplitude scaling, which enables users to build the index to process the query. We propose a new index structure, KV-index, and the matching algorithm, KV-match. With a single index, our approach can support both RSM and cNSM problems under either ED or DTW distance. KV-index is a key-value structure, which can be easily implemented on local files or HBase tables. To support the query of arbitrary lengths, we extend KV-match to KV-match$_{DP}$, which utilizes multiple varied-length indexes to process the query. We conduct extensive experiments on synthetic and real-world datasets. The results verify the effectiveness and efficiency of our approach.

==> tex/dynamic1.tex <==
\section{KV-\MakeLowercase{match}$_{\text{DP}}$}%: Extending KV-\MakeLowercase{match} \newline with Multi-Level Indexes}
\label{sec:dynamic}
%In this section, we introduce KV-match$_{DP}$, which uses a set of indexes with variable window lengths.

%\needspace{1cm}
%\subsection{Single Index is Not Optimal}
The basic KV-match uses a fixed window length $w$ to process the query, regardless of the query length. It has two limitations. First, the length of the supported query is limited. %If $w$ is too large, query with length smaller than $w$ can not be processed. If $w$ is too small, we need to process many disjoint windows for long queries.
Second, we have less chance to exploit the characteristics of the query and the time series data to speed up processing. %For example, assume $Q$ contains a length-30 subsequence which is a burst, and the mean value of this subsequence is very rare in time series $X$, so a shorter disjoint window of length-30 may be better placed here. In the meanwhile, $Q$ also contains a length-100 stable subsequence which is unusual, and a length-100 disjoint window can result in a very small candidate set. If the query series is segmented into fixed-length disjoint windows, these characteristics cannot be utilized together. %Our experiment also demonstrates this issue, which can be seen in Figure~\ref{fig:exp7}.

In this section, we propose KV-match$_{\text{DP}}$, which is based on multiple indexes with variable window lengths. Formally, the lengths of windows to build the index are summarized by two parameters, $w_u$ and $L$, where $w_u$ is the minimum window length and $L$ is the number of indexes. Then, the set of window lengths is $\Sigma=\{w_u * 2^{i-1} | 1 \leq i \leq L\}$. For example, suppose $w_u=25$ and $L=5$, we build indexes of length $25$, $50$, $100$, $200$ and  $400$ respectively. We use KV-index$_w$ to denote the index based on length-$w$ windows.
%Let KV-index$_w$ represent the index based on length-$w$ windows.
%The corresponding indexes are denoted as KV-index$_{w_u*2^{i-1}}$ ($1\leq i\leq L$) respectively.
%Since KV-index is built by sequentially scanning the time series,
The set of indexes can be built simultaneously by extending the index building algorithm in Section~\ref{sec:index_building_algorithm} easily.


\subsection{Dynamic Query Segmentation}
We process the query with multiple indexes simultaneously. That is, we split $Q$ into a sequence of disjoint windows of variable lengths, $\{Q_1, Q_2,\cdots, Q_p\}$, and process each $Q_i$ with KV-index$_{|Q_i|}$, which is more flexible to utilize the characteristics of the data.
%Note that value $p$ may be different when $Q$ varies.
Once $Q$ is split, the following process is similar to that in KV-match. The only difference is that for window $Q_i$, we fetch $\textit{RList}_i$ from index KV-index$_{|Q_i|}$. Note that although in Lemmas in Section~\ref{sec:motivation}, $Q$ is split into equal-length windows, we can easily extend them to variable-length windows, since the proof always involves only one window.

The challenge here is how to split query $Q$ to achieve the best performance. We use \emph{query segmentation} to represent the result of query splitting. A segmentation, denoted as $\textit{SG}=\{r_1, r_2, \cdots, r_p\}$, means that $Q_1=Q(1,r_1)$, $Q_2=Q(r_1+1,r_2-r_1)$ and so on.
%Note that even for two queries of equal length, the number of disjoint windows may be also different.
A high-quality segmentation should satisfy: 1) the length of each window belongs to $\Sigma$; 2) processing $Q$ with these windows results in high performance. %In this paper,
We take the segmentation as an optimization problem and design an objective function to measure its quality.%, and propose a two-dimensional dynamic programming algorithm to solve it.


\needspace{10mm}
\subsection{The Objective Function}
%Before introducing the objective function,
We first analyze the key factors to impact the efficiency. The runtime of query processing $T$ is composed of $T_1$ and $T_2$, those of phase 1 and 2 respectively. %As shown in Figure~\ref{fig:exp5-1}, the fluctuation range of $T_2$ is much larger than $T_1$. So
According to our theoretical analysis and experimental verification, $T_2$ is more significant to the efficiency, % A poor-quality segmentation may make phase 2 very slow.
while $T_1$ is more stable. So we utilize the efficiency of phase 2 to measure the segmentation quality. Phase 2 consists of two parts, data fetching and distance computation, the former of which, determined by $n_I(\textit{CS})$, is much more time-consuming.

Therefore, for a segmentation $\textit{SG}$ of $Q$, after obtaining the final candidate set $\textit{CS}$, we use $n_I(\textit{CS})$ to measure the quality of $\textit{SG}$. The smaller $n_I(\textit{CS})$, the higher quality of $\textit{SG}$.
%So we hope to find the optimal segmentation with the smallest value of $n_I(CS)$.
The challenge is we cannot obtain the exact value of $n_I(\textit{CS})$ without going through the index-probing phase. Moreover, although we can obtain the size of $n_I(\textit{CS}_i)$'s from the meta table, we cannot compute $n_I(\textit{CS})$ with $n_I(\textit{CS}_i)$'s directly.

To address this issue, we propose an objective function to estimate the value of $n_I(\textit{CS})$. The estimation is based on two assumptions. First, $\textit{IS}_i$'s of disjoint windows are independent with each other ($1\leq i \leq p$). Second, the size of each window interval in $\textit{IS}_i$ is much smaller than $|X|$. So we can take each window interval as a single point in $X$, and these positions are distributed uniformly.

Next, we introduce our objective function, denoted as $\mathcal{F}$. Assume that we use $\textit{SG}$ to split $Q$ into $Q_1, Q_2, \cdots, Q_p$, and obtain the size of each $\textit{IS}_i$ ($1\leq i\leq p$) based on the meta table. Then we estimate $n_I(\textit{CS})$ as follows. Based on these two assumptions, we can use $\frac{n_I(\textit{IS}_1)}{n}$ to approximately represent the probability of an interval contained in $\textit{CS}_1$, where $n$ is the length of $X$. It follows that $\frac{n_I(\textit{IS}_1)}{n} * \frac{n_I(\textit{IS}_2)}{n}$ is the probability of an interval contained in $\textit{CS}_1 \cap \textit{CS}_2$. Therefore, $\prod_{i=1}^{p}\frac{n_I(\textit{IS}_i)}{n}$ is the probability of an interval contained in the final $\textit{CS}$, which is proportional to $n_I(\textit{CS})$. It is obvious that the larger $p$, the smaller $\prod_{i=1}^{p}\frac{n_I(\textit{IS}_i)}{n}$. So, to eliminate the effect of number of windows, we take geometric mean of this value as the final objective function $\mathcal{F}$, as follows,

\small
\begin{equation}
	\mathcal{F}(\textit{SG}) = \sqrt[\leftroot{0}\uproot{25}p]{\prod_{i=1}^{p}\frac{n_I(\textit{IS}_i)}{n}} = \frac{1}{n}\sqrt[\leftroot{0}\uproot{25}p]{\prod_{i=1}^{p} n_I(\textit{IS}_i)}
	\label{eq:objection_function}
\end{equation}
\normalsize
%where $n_I(IS_i)$ can be obtained directly from the meta table.

The target segmentation is the one with the minimal value of $\mathcal{F}$\footnote{Since $\frac{1}{n}$ is a constant, we ignore it in the algorithm.}.

\subsection{Two-dimensional DP Approach}
%Given the objective function $J$,
We propose a two-dimensional dynamic programming algorithm to find the optimal $\textit{SG}$. We first define the search space. Since the length of each window $Q_i$ must belong to $\Sigma$, so in any $\textit{SG}=\{r_1, r_2,\cdots, r_p\}$, $r_i$ must be multiple times of $w_u$. Any $\textit{SG}$ not satisfying this constraint is invalid. Given query $Q=(q_1,q_2,\cdots,q_{m})$, we define the search space with sequence $Z=(1, 2,\cdots, m')$, where $m'=\lfloor\frac{m}{w_u}\rfloor$. Note that the values in $Z$ do not have impact on the generation of $\textit{SG}$. The only effect of $Z$ is to constrain the search space of $\textit{SG}$. Instead of finding $\textit{SG}$ on $Q$ directly, we find it from $Z$, denoted as $\textit{SG}_Z$, and then map it to $\textit{SG}$ of $Q$ by multiplying each endpoint of $Z$ with $w_u$. For example, let $|Q|=200$, $w_u=25$ and $L=3$. That is, we have three indexes, KV-index$_{25}$, KV-index$_{50}$ and KV-index$_{100}$. $\textit{SG}_Z=\{2, 6, 7, 8\}$ corresponds to $\textit{SG}=\{50, 150, 175, 200\}$. In this case, $Q$ is segmented into four windows, $Q(1,50)$, $Q(51,100)$, $Q(151,25)$ and $Q(176,25)$.

We search the optimal $\textit{SG}_Z$ with two-dimensional dynamic programming from left to right on $Z$ sequentially. The first dimension represents the boundaries of segmentation, and the second represents the number of windows contained in a segmentation. We use $v_{i,j}$ to represent a sub-state of calculation process, which corresponds to the best segmentation of the prefix of $Z$, $Z(1, i)$, with $j$ number of windows. For any $j$ ($1 \leq j \leq m'$), the best segmentation is the one with minimum $v_{m',j}$. After obtaining all $v_{m',j}$'s, we select the minimal one as the final $\textit{SG}_Z$, and map it to $\textit{SG}$.
The dynamic programming equation is presented as Eq.~(\ref{eq:dp}).

In Eq.~(\ref{eq:dp}), $\varphi$ represents the possible lengths of the window ending at $i$ in $\textit{SG}_Z$, and it has $L$ possible values at most. $C_{i-\varphi+1, \varphi}$ is the value of $n_I(\textit{IS})$ for the disjoint window $Q((i-\varphi)*w_u+1,\varphi *w_u)$, which can be obtained from the meta table of KV-index$_{\varphi *w_u}$, as explained in Section~\ref{sec:matching}.
The optimal $\textit{SG}_Z$ and $\textit{SG}$ can be recovered by leveraging backward-pointers. Due to space limitation, we provide the complete pseudo-code in our longer paper~\cite{arxiv}.% The complete algorithm is shown in Algorithm~\ref{alg:dp}.

\vspace{-4mm}
\small
\begin{equation}
	v_{i,j}= \left\{
	\begin{array}{l@{\;,\;}l}
	1 & i=0 \wedge j=0 \\
	%+\infty & i=0 \wedge j \neq 0 \\
	+\infty & i = 0 \vee j = 0 \\
	\displaystyle\min_{\mathclap{\substack{\varphi=2^{k-1} \\ \mathmakebox[130\fboxrule][r]{1} \leq k \leq \min(L, \log_2(i)+1)}}}
		\sqrt[\leftroot{-3}\uproot{8}j]{(v_{i-\varphi, j-1})^{j-1} * C_{i-\varphi+1, \varphi}} & 1 \leq j \leq i \leq m'
	\end{array}
	\right.
	\label{eq:dp}
\end{equation}
\normalsize

\vspace{-1mm}
%\begin{algorithm}[t]
%	\small
%	\caption{Segment($w_u, L, Q$)}
%	\begin{algorithmic}[1]
%		\State $m' \gets \left\lfloor\frac{|Q|}{w_u}\right\rfloor, v_{i,j} \gets +\infty, P_{i,j} \gets -1$ $(0 \leq i \leq m')$ \label{alg3:initial:begin}
%		\State $v_{0,0} \gets 1$ \label{alg3:initial:end}
%		\For {$i \gets 1, m'$} \label{alg3:dp:begin}
%			\For {$j \gets 1, i$}
%				\For {$k \gets 1, \min(L, \log_2(i)+1)$}
%					\State $\varphi \gets 2^{k-1}$
%					\If {$\sqrt[\leftroot{-3}\uproot{8}j]{(v_{i-\varphi, j-1})^{j-1} * C_{i-\varphi+1, \varphi}} < v_{i,j}$}
%						\State $v_{i,j} \gets \sqrt[\leftroot{-3}\uproot{8}j]{(v_{i-\varphi, j-1})^{j-1} * C_{i-\varphi+1, \varphi}}$
%						\State $P_{i,j} \gets \varphi$
%					\EndIf
%				\EndFor
%			\EndFor
%		\EndFor \label{alg3:dp:end}
%		\State $SG \gets \varnothing, i \gets m', j \gets \underset{x}{\arg\min}(v_{m', x})$ $(1 \leq x \leq m')$ \label{alg3:recover:begin}
%		\While {$i \neq -1$}
%			\State $SG$.add($i * w_u$)
%			\State $i \gets i - P_{i,j}, j \gets j - 1$
%		\EndWhile \label{alg3:recover:end}
%		\State \Return $SG$	
%	\end{algorithmic}
%	\label{alg:dp}
%\end{algorithm}

\emph{Analysis.} It happens that a large amount of windows of $X$ have similar mean values. In this case, certain rows in KV-index will have large value of $n_I$, which incurs large I/O cost to fetch $RList$ and large computation cost to merge $CS_i$ in each round. The KV-index$_{\text{DP}}$ can alleviate this phenomenon to some extent, since the objective function prefer the query windows with smaller $n_I$.

Moreover, we can use some techniques to alleviate this phenomenon further. First, to reduce the duplicate index visit, we can cache the index rows already fetched. Then for each new $RList$, if partial of it is already in the cache, we only need to fetch the rest part from KV-index. Second, we can reorder  $Q_i$'s to be processed according to the size of $RList_i$, which can be obtained easily from the meta data. In other words, we first process $Q_i$ with smaller $RList_i$, which can reduce both I/O cost and the merge computation cost. Third, note that each $CS_i$ is the \emph{superset} of the true result, so we can only process a partial of query windows, instead of all of them, to obtain the final $CS$ without loss of correctness. By combining the second and third optimization, we can skip some rows with large $n_I$ by ranking them at the bottom position.


==> tex/experiment.tex <==
\needspace{10mm}
\section{Experiments}
\label{sec:experiment}
In this section, we conduct extensive experiments to verify the effectiveness and efficiency of the proposed approach.

\subsection{Datasets and Settings}

\subsubsection{Real Datasets}
UCR Archive~\cite{UCRArchive} is a popular time series repository, which includes many datasets widely used in time series mining research. We concatenate the time series in UCR Archive to obtain desired length time series.

\subsubsection{Synthetic Datasets}
We use synthetic time series to test the scalability of our approach. The series are generated by combining three types of time series as follows.
\begin{itemize}
	\item Random walk. The start point and step length are picked randomly from $[-5, 5]$ and $[-1, 1]$ respectively;
	\item Gaussian. The values are picked from a Gaussian distribution with mean value and standard deviation randomly selected from $[-5, 5]$ and $[0, 2]$ respectively;
	\item Mixed sine. It is a mixture of several sine waves whose period, amplitude and mean value are randomly chosen from $[2, 10]$, $[2, 10]$ and $[-5, 5]$ respectively.
\end{itemize}

To generate a time series $X$, we execute the following steps repeatedly until $X$ is fully generated: i) randomly choose a type $t$, a length $l$ and the parameters according to type $t$; ii) generate a length-$l$ subsequence using type $t$ with parameters.

\subsubsection{Implementation}
We implement two versions of our approach to show the compatibility of our approach, a local disk version, and an HBase version. Both are implemented with Java. The code is publicly available\footnote{https://github.com/DSM-fudan/KV-match}.

In local disk version, The index is stored as a local file, which consists of two parts, index part and meta part. In the index part, the ordered rows, $\{(K_1,V_i),(K_2,V_2),\cdots\}$, are stored contiguously. The meta part maintains the lists of the quadruples, $\left<K_i, pos_i, n_I(V_i), n_P(V_i)\right>$ ($i=1,2,\cdots$), where $pos_i$ is the offset of the $i$-th row in the file. During query processing, The start and end row offset of each scan operation can be inferred by binary search on meta data, then a seek operation is used to fetch corresponding rows.

To verify the scalability of KV-match, we implement it on HBase~\cite{hbase}. Two HBase tables are created, one data table and one index table, both of which have a single column family. In the data table, time series is split into equal-length (1024 by default) disjoint windows, and each one is stored as a row. The key is the window position, and the value is the corresponding subsequence. In index table, each row of KV-index is stored as a row in HBase, $K_i$ as the key and $V_i$ as the value. The meta table is also compacted to store as a row in index table. We use the ``scan'' API of HBase to fetch $RList$ directly.

%We load the meta table to memory before processing the query. %To take full advantage of the cluster, we adapt index building algorithm to the MapReduce framework.


\subsubsection{Counterpart Approaches}
For RSM, we compare our approach (\textit{KVM} for short) with two index-based approaches, General Match~\cite{gmatch02} for ED and DMatch~\cite{Fu2008} for DTW. For cNSM, we compare with UCR Suite~\cite{kdd12} and FAST~\cite{edbt17}.

General Match~\cite{gmatch02} (\textit{GMatch} for short) is a classic R*-tree based approach for ED. We use the code from author, which
%is implemented in C and
stores indexes in local disk files. Since building and updating R*-tree in distributed environment is not straightforward, we only compare it with our local file version. %General Match has two parameters, $J$ and $w$. We use the optimal value as mentioned in its paper.

DMatch~\cite{Fu2008} is a duality-based subsequence matching approach for DTW, which is quite similar to other tree-style approaches. Because its code is not publicly available, we implement a C++ version based on General Match framework. The window length is set to 64 and each window is transformed to a 4-dimensional point by PAA. %Note that, it is not Dual Match~\cite{dualmatch01}, which transforms windows by DFT.

UCR Suite~\cite{kdd12} (\textit{UCR} for short) finds the best normalized matching subsequence under both ED and DTW. It scans the whole time series data, and uses some lower-bound techniques to speed up the query processing. Its code is publicly available\footnote{http://www.cs.ucr.edu/\raise.17ex\hbox{$\scriptstyle\sim$}eamonn/UCRsuite.html}, which is implemented in C++ and reads data on local disks. To make the comparison fair, we alter it to $\varepsilon$-match problem. Moreover, we implement a Java version to retrieve data on HBase, and conduct experiments for both local file and HBase table version to compare its scalability with KV-match.

FAST~\cite{edbt17} is a recent improvement on UCR Suite, which adds more lower-bound techniques to reduce the number of distance calculations. We use the code from author, and compare it with our local file version under both ED and DTW.

%\needspace{5mm}
\subsubsection{Default Setting}
In KV-match$_{\text{DP}}$, $L$ is set to 5, and $\Sigma = \left\{25, 50, 100, 200, 400\right\}$. In index building algorithm, the initial fixed width $d$ is set to $0.5$ and the merge threshold $\gamma$ is set to $80\%$.
%Except the experiments to verify the effectiveness of the window reduction and reordering, all proposed techniques are used.
All experimental results are averaged over 100 runs.
The parameters $d$ and $\gamma$ do not effect the performance greatly. So we omit the experimental results of these parameters. Interested reader can find it in our longer paper~\cite{arxiv}.

%Similar to other tree-based approaches, we also evaluate the performance of our approach under different selectivities. The selectivity is the ratio between the number of qualified subsequences and that of all possible subsequences, $|X|-|Q|+1$. We generate query series by extracting subsequences of $X$ starting from random offsets.

To test the performance of processing queries with arbitrary lengths, we generate queries of length $128, 256, \cdots, 8192$. For each length, 100 different query series are generated. 

%We obtain the desired selectivity by controlling the threshold $\varepsilon$ and uniformly distributing query series over various selectivities in the given range. For cNSM problem, we collect queries for each $\left<\alpha, \beta\right>$ pair under particular selectivity by controlling $\varepsilon$.

Experiments are executed on a cluster consisting of 8 nodes with HBase 1.1.5 (1 Master and 7 RegionServers). Each node is powered by Linux, and has two Intel Xeon E5 1.8GHz CPUs, 64GB memory, 5TB HDD storage. Experiments using local file version are executed on a single node of the cluster.


\begin{table}[t]
	\centering
	\caption{Results of RSM Queries Under ED Measure}
	\label{tab:exp1-ed}
	\begin{tabular}{@{\extracolsep{4pt}}ccrrr@{}}
		\hline
		\multirow{2}{*}{\textbf{Approach}} & \multirow{2}{*}{\textbf{Selectivity}} & \multirow{2}{*}{\textbf{\#candidates}} & \textbf{\#index} & \multirow{2}{*}{\textbf{Time} (ms)} \\
		& & & \textbf{accesses} & \\
		\hline
		& \textbf{$\bm{10^{-9}}$} &        13.9 & 279.2 &    852.3 \\
		&	\textbf{$\bm{10^{-8}}$} &      1837.5 & 240.1 &    541.2 \\
		\textbf{GMatch}   & \textbf{$\bm{10^{-7}}$} &   239,857.4 & 226.2 &  5,817.5 \\
		& \textbf{$\bm{10^{-6}}$} & 1,223,370.6 & 338.0 & 30,351.7 \\
		& \textbf{$\bm{10^{-5}}$} & 1,410,563.0 & 313.6 & 34,916.4 \\
		\hline
		& \textbf{$\bm{10^{-9}}$} &     2,754.9 &   4.6 &     60.4 \\
		&	\textbf{$\bm{10^{-8}}$} &     6,313.2 &   4.5 &     70.8 \\
		\textbf{KVM-DP}   & \textbf{$\bm{10^{-7}}$} &    29,853.1 &   4.4 &    138.8 \\
		& \textbf{$\bm{10^{-6}}$} &   113,434.1 &   6.0 &    567.4 \\
		& \textbf{$\bm{10^{-5}}$} &   153,565.1 &   7.0 &  1,200.7 \\
		\hline
	\end{tabular}
\end{table}

\begin{table}[t]
	\centering
	\caption{Results of RSM Queries Under DTW Measure}
	\label{tab:exp1-dtw}
	\begin{tabular}{@{\extracolsep{4pt}}ccrrr@{}}
		\hline
		\multirow{2}{*}{\textbf{Approach}} & \multirow{2}{*}{\textbf{Selectivity}} & \multirow{2}{*}{\textbf{\#candidates}} & \textbf{\#index} & \multirow{2}{*}{\textbf{Time} (ms)} \\
		& & & \textbf{accesses} & \\
		\hline
		& \textbf{$\bm{10^{-9}}$} & 1,176,639.8 & 250.0 &     543.5 \\
		&	\textbf{$\bm{10^{-8}}$} & 1,278,894.9 & 276.1 &   1,424.2 \\
		\textbf{DMatch}   & \textbf{$\bm{10^{-7}}$} & 1,800,014.9 & 447.8 &   7,847.2 \\
		& \textbf{$\bm{10^{-6}}$} & 2,406,697.3 & 619.2 &  29,952.9 \\
		& \textbf{$\bm{10^{-5}}$} & 3,431,349.8 & 902.9 & 132,062.4 \\
		\hline			
		& \textbf{$\bm{10^{-9}}$} &  25,423.9 &   4.7 &    115.3 \\
		&	\textbf{$\bm{10^{-8}}$} &  38,894.0 &   4.9 &    120.5 \\
		\textbf{KVM-DP}   & \textbf{$\bm{10^{-7}}$} &  87,002.5 &   5.3 &    634.1 \\
		& \textbf{$\bm{10^{-6}}$} & 118,580.9 &   6.6 &  3,641.3 \\
		& \textbf{$\bm{10^{-5}}$} & 218,965.5 &   7.1 & 21,348.2 \\
		\hline
	\end{tabular}
\end{table}
\begin{table}[t]
	\centering
	\caption{Results of cNSM Queries Under ED Measure}
	\label{tab:exp2-ed}
	%\small
	\begin{tabular}{@{\extracolsep{3.5pt}}clrrrrr@{}}
		\hline
		\multirow{2}{*}{\textbf{Selectivity}} & \multicolumn{4}{c}{\textbf{KVM-DP} (s)} & \multicolumn{1}{c}{\textbf{UCR}} & \multicolumn{1}{c}{\textbf{FAST}} \\
		\cline{2-5}\cline{6-6}\cline{7-7}
		& \multicolumn{1}{c}{$\bm{\alpha}$\textbackslash $\bm{\beta'}$} & \multicolumn{1}{c}{\textbf{1.0}} & \multicolumn{1}{c}{\textbf{5.0}} & \multicolumn{1}{c}{\textbf{10.0}} & \multicolumn{1}{c}{\textbf{Avg.(s)}} & \multicolumn{1}{c}{\textbf{Avg.(s)}}\\
		\hline
		\multirow{3}{*}{$\bm{10^{-9}}$}  & \textbf{1.1} & 0.51 & 2.33 & 4.64 & \multirow{3}{*}{59.84} & \multirow{3}{*}{86.05}\\ %\cline{2-6}
		& \textbf{1.5} & 0.56 & 2.58 & 5.05 &\\ %\cline{2-6}
		& \textbf{2.0} & 0.59 & 2.70 & 5.51 &\\
		\hline
		\multirow{3}{*}{$\bm{10^{-8}}$}  & \textbf{1.1} & 0.72 & 3.22 & 6.18 & \multirow{3}{*}{60.17} & \multirow{3}{*}{86.09}\\ %\cline{2-6}
		& \textbf{1.5} & 1.00 & 4.60 & 8.98 &\\ %\cline{2-6}
		& \textbf{2.0} & 1.22 & 5.47 & 10.66 &\\
		\hline
		\multirow{3}{*}{$\bm{10^{-7}}$} & \textbf{1.1} & 1.30 & 5.46 & 10.29 & \multirow{3}{*}{65.25} & \multirow{3}{*}{87.79}\\ %\cline{2-6}
		& \textbf{1.5} & 2.82 & 11.53 & 21.75 &\\ %\cline{2-6}
		& \textbf{2.0} & 3.72 & 16.20 & 29.15 &\\
		\hline
		\multirow{3}{*}{$\bm{10^{-6}}$} & \textbf{1.1} & 1.69 & 6.74 & 14.53 & \multirow{3}{*}{69.17} & \multirow{3}{*}{88.64}\\ %\cline{2-6}
		& \textbf{1.5} & 3.15 & 15.19 & 27.53 &\\ %\cline{2-6}
		& \textbf{2.0} & 4.39 & 20.77 & 35.75 &\\
		\hline
		\multirow{3}{*}{$\bm{10^{-5}}$} & \textbf{1.1} & 1.94 & 7.82 & 12.92 & \multirow{3}{*}{70.59} & \multirow{3}{*}{89.83}\\ %\cline{2-6}
		& \textbf{1.5} & 4.23 & 15.98 & 28.26 &\\ %\cline{2-6}
		& \textbf{2.0} & 5.77 & 21.55 & 37.66 &\\
		\hline
	\end{tabular}
\end{table}

\begin{table}[t]
	\centering
	\caption{Results of cNSM Queries Under DTW Measure}
	\label{tab:exp2-dtw}
	%\small
	\begin{tabular}{@{\extracolsep{1.5pt}}clrrrrr@{}}
		\hline
		\multirow{2}{*}{\textbf{Selectivity}} & \multicolumn{4}{c}{\textbf{KVM-DP} (s)} & \multicolumn{1}{c}{\textbf{UCR}} & \multicolumn{1}{c}{\textbf{FAST}}  \\
		\cline{2-5}\cline{6-6}\cline{7-7}
		& \multicolumn{1}{c}{$\bm{\alpha}$\textbackslash $\bm{\beta'}$} & \multicolumn{1}{c}{\textbf{1.0}} & \multicolumn{1}{c}{\textbf{5.0}} & \multicolumn{1}{c}{\textbf{10.0}} & \multicolumn{1}{c}{\textbf{Avg.(s)}} & \multicolumn{1}{c}{\textbf{Avg.(s)}} \\
		\hline
		\multirow{3}{*}{$\bm{10^{-9}}$}  & \textbf{1.1} & 0.72 & 2.71 & 3.71 & \multirow{3}{*}{139.57} & \multirow{3}{*}{77.5}\\ %\cline{2-6}
		& \textbf{1.5} & 0.66 & 2.97 & 4.72 &\\ %\cline{2-6}
		& \textbf{2.0} & 0.78 & 3.37 & 6.00 &\\
		\hline
		\multirow{3}{*}{$\bm{10^{-8}}$} & \textbf{1.1} & 0.89 & 2.66 & 5.31 & \multirow{3}{*}{140.06} & \multirow{3}{*}{78.57}\\ %\cline{2-6}
		& \textbf{1.5} & 1.24 & 4.89 & 7.89 &\\ %\cline{2-6}
		& \textbf{2.0} & 1.43 & 5.01 & 9.21 &\\
		\hline
		\multirow{3}{*}{$\bm{10^{-7}}$} & \textbf{1.1} & 1.88 & 6.61 & 10.02 & \multirow{3}{*}{142.99} & \multirow{3}{*}{85.07}\\ %\cline{2-6}
		& \textbf{1.5} & 3.81 & 13.79 & 23.30 &\\ %\cline{2-6}
		& \textbf{2.0} & 4.46 & 15.92 & 33.00 & \\
		\hline
		\multirow{3}{*}{$\bm{10^{-6}}$} & \textbf{1.1} & 5.58 & 14.29 & 18.69 & \multirow{3}{*}{153.88} & \multirow{3}{*}{103.60}\\ %\cline{2-6}
		& \textbf{1.5} & 11.09 & 30.74 & 60.27 &\\ %\cline{2-6}
		& \textbf{2.0} & 11.40 & 33.72 & 60.56 &\\
		\hline
		\multirow{3}{*}{$\bm{10^{-5}}$} & \textbf{1.1} & 19.75 & 36.61 & 49.94 & \multirow{3}{*}{177.28} & \multirow{3}{*}{137.01}\\ %\cline{2-6}
		& \textbf{1.5} & 40.35 & 57.90 & 102.72 &\\ %\cline{2-6}
		& \textbf{2.0} & 44.07 & 76.23 & 106.97 &\\
		\hline
	\end{tabular}
\end{table}

\subsection{Results of RSM Queries}
\label{sec:experiment_gmatch}
We first compare KV-match$_{\text{DP}}$ with General Match and DMatch. The experiment is conducted on length-$10^9$ real dataset with queries of different selectivities. The results are shown in Table~\ref{tab:exp1-ed} and \ref{tab:exp1-dtw} respectively. 
%We report the number of candidates, the number of index accesses and the runtime.

It can be seen that when the selectivity increases, the number of candidates of General Match explodes dramatically, and in the case of higher selectivities, it is much larger than that of ours. Although General Match converts all values in a window into a multi-dimensional point, which keeps more information than the mean value used in KV-index, it generates candidates only based on one single window. In contrast, our approach combines the pruning power of multiple windows, which can achieve smaller candidate set. %Especially when the query length and the threshold $\varepsilon$ increases, the single window mechanism of General Match incurs many false candidates.

The number of index accesses of General Match is 20-30 times larger than that of ours. Due to fewer index accesses and less number of candidates, our approach achieves the overall performance improvement of one order of magnitude compared to General Match. An interesting phenomenon is that for queries of low selectivities ($10^{-8}$ or $10^{-9}$), the number of candidates of our approach is slightly larger than that of General Match. However, benefiting from fewer index accesses, we still achieve better overall performance.


Similar to General Match, DMatch also conducts large number of index accesses, and has to verify one or two orders of magnitude more candidates than ours. The reason is still the single window candidate generation mechanism and tree-style index structure, as General Match. %As a result, our approach achieves the overall performance improvement of one to two orders of magnitude.

\subsection{Influence of Window Size $w$}
In this experiment, we investigates the pruning performance of building index with the mean values. We compare the number of candidates obtained from each query window $Q_i$ of KV-match and FRM~\cite{frm94}~\footnote{FRM is a special case of General Match when $J=1$.}. FRM is selected to compare because its mechanism is analogous to KV-match. FRM builds the index based on the sliding windows of $X$, and each window is transformed into an $f$-dimensional point. Then the transformed points are stored in R-tree. To process query $Q$, FRM splits $Q$ into $p$ number of disjoint windows $Q_i$ ($1\leq i\leq p$). For each window, a set of candidates are obtained by a range query to R-tree. Then, the \emph{union} of candidates of all windows forms the final candidate set. In contrast, in KV-match, the final candidate sets, $CS$, is the intersection of $CS_i$'s.

In Table~\ref{tab:win-total-candidates-small}, we show the ratio of number of candidates per window between our approach and FRM. The experiments are conducted on time series of length $10^9$. We run queries of different selectivities. For each selectivity, 100 randomly generated queries of length 2048 are processed, and the number of candidates are averaged. We compare KV-indexes and FRM with variable window sizes, 50, 100, 200, 400. Moreover, we also show the ratio of the number of final candidates between our approach and FRM. Due to the space limit, we only list the results of query of length 2048. More results of multiple query lengths can be found in the longer version~\cite{arxiv}.

It can be seen that our approach will generate more candidates per window, $CS_i$, especially for smaller $w$ and larger $|Q|$, since the range depends on $\frac{\varepsilon}{w}$. However, the number of final candidates, $CS$, of our approach is much smaller than that of FRM, because in KV-match, $CS$ is the intersection of $CS_i$'s, while in FRM, $CS$ is the union of $CS_i$'s. Consider it is more expensive to fetch the time series to compute the distance, reducing $CS$ is more beneficial. Moreover, for each $Q_i$, we only visit index with a sequential scan operation, while in FRM we need to visit multiple index nodes, which may incur more I/O cost. Finally, the mechanism of KV-match${_{\text{DP}}}$ can avoid to use the query windows with many candidates.

\begin{table}[t]
	\centering
	\caption{The Ratio of KV-match and FRM on Window Averaged Candidates vs. Final Total Candidates $(Len(Q)=2048)$}
	\label{tab:win-total-candidates-small}
	%\small
	\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}crrrrrr@{}}
		\hline
		\multirow{2}{*}{\textbf{Selectivity}} & \multicolumn{3}{c}{\textbf{Window averaged}} & \multicolumn{3}{c}{\textbf{Final total}} \\
		\cline{2-4}\cline{5-7}
		& \multicolumn{1}{c}{$\bm{w=}$ \textbf{50}} & \multicolumn{1}{c}{\textbf{100}} & \multicolumn{1}{c}{\textbf{400}} & \multicolumn{1}{c}{$\bm{w=}$ \textbf{50}} & \multicolumn{1}{c}{\textbf{100}} & \multicolumn{1}{c}{\textbf{400}} \\
		\hline
		\multirow{1}{*}{$\bm{10^{-6}}$}	&  52.1 &  65.5 &  21.2 & 0.010 & 0.007 &   0.323 \\		
		\multirow{1}{*}{$\bm{10^{-5}}$} &  41.0 &  18.4 &  10.2 & 0.209 & 0.076 &   0.040 \\		
		\multirow{1}{*}{$\bm{10^{-4}}$} &  62.3 &  23.0 &   5.7 & 0.483 & 0.181 &   0.071 \\
		\multirow{1}{*}{$\bm{10^{-3}}$} &  68.5 &  26.1 &   5.2 & 0.531 & 0.319 &   0.152 \\
		\hline
	\end{tabular*}
\end{table}

\begin{table}[t]
	\centering
	\caption{Influence of $w$ on Index Size and Building Time}
	\label{tab:w-index}
	\begin{tabular*}{0.6\linewidth}{@{\extracolsep{\fill}}crr@{}}
		\hline
		$\bm w$ & \textbf{Size (MB)} & \textbf{Building time (s)} \\
		\hline
		\textbf{25}	 & 354.09 & 299.38 \\
		\textbf{50}	 & 287.21 & 234.30 \\
		\textbf{100} & 236.49 & 227.06 \\
		\textbf{200} & 194.52 & 210.18 \\
		\textbf{400} & 155.47 & 198.12 \\
		\hline
	\end{tabular*}
\end{table}

\subsection{Results of cNSM Queries}
In this experiment, we compare KV-match$_{\text{DP}}$ with UCR Suite and FAST for cNSM on local disk. The experiment is conducted on length-$10^9$ real dataset with queries of different selectivities. The results under ED and DTW measures are shown in Table~\ref{tab:exp2-ed} and \ref{tab:exp2-dtw} respectively. For each selectivity, we report the runtime for different $\alpha$ and $\beta$. The constraints are also embedded into UCR Suite and FAST, so unqualified candidates are abandoned too. For simplicity, we only report the average runtime for each selectivity, because theirs runtime for queries in the same selectivity group is quite similar.

We use relative offset shifting $\beta'$ in cNSM experiments, which is the percentage of the value range of the whole data series. Therefore, $\beta=(\max(X)-\min(X))* \beta'\%$.

It can be seen that when the selectivity increases, the runtime of KV-match increases steadily. When the selectivity is fixed, the runtime increases as $\alpha$ and $\beta$ increase. Because UCR Suite almost always scans the whole dataset, its runtime is more stable and dominated by I/O cost. The extra lower-bounds in FAST seems not efficient for ED, due to its overhead of data preparation. While for DTW, FAST achieves obvious improvement comparing to UCR Suite, especially for queries of low selectivities ($10^{-8}$ or $10^{-9}$). In most cases, our approach achieves the performance improvement of one to two orders of magnitude compared to them. %In worst cases, UCR Suite needs 90.55s for ED and 228.57s for DTW queries.

%UCR-DTW: 138.56s -- 228.57s

\subsection{Index Size and Building Time}
\label{sec:experiment_size}
We compare the index space cost and building time of KV-match$_{\text{DP}}$ and DMatch. GMatch has similar space cost and building time as those of DMatch, and so we do not show them in the results. The experiment is conducted on the local file version with real datasets. Results are shown in Fig.~\ref{fig:exp6}.
We also show the size of time series data as dark blue bars.

It can be seen that the index sizes of both DMatch and KV-match$_{\text{DP}}$ are about 10\% of data size, and the size of KV-match$_{\text{DP}}$ is slightly larger than that of DMatch. However, KV-match$_{\text{DP}}$ consists of 5 KV-indexes, so the size of a single KV-index is much smaller than that of DMatch. We also show the index building time as lines in Fig.~\ref{fig:exp6}. Our index is much more efficient to build, due to its simple structure. In the extremely large data scale (the trillion-length time series), it takes 36 hours to build all 5 KV-indexes for KV-match$_{\text{DP}}$ on HBase.

Moreover, we test the influence of window size $w$ on the index size and building time. In Table~\ref{tab:w-index}, we show the index size and building time of KV-index with fixed $w$ on time series of length $10^9$. It can be seen that as $w$ increases, both index size and building time decrease gradually. This is because that larger $w$ makes the mean values of the adjacent windows more similar, and correspondingly makes $n_I(V_i)$ smaller, which reduces both the index size and the building time.

%UCR-ED: 59.64s -- 90.55s



\subsection{Scalability}
To investigate the scalability of our approach, we use longer synthetic time series, from length-$10^9$ to length-$10^{12}$, to compare KV-match$_{\text{DP}}$ and UCR Suite for cNSM queries. Both time series data and our index is stored as HBase table, and both ED and DTW measures are compared. We set $\alpha=1.5$, $\beta'=1.0$, and hold selectivity to $10^{-7}$ by adjusting $\varepsilon$. The results are shown in Fig.~\ref{fig:exp2}.

\begin{figure}[t]
	\begin{minipage}[t]{0.49\linewidth}
		\includegraphics[width=40mm,height=30mm]{figure/exp6-size-time.eps}
		\caption{Size \& building time}
		\label{fig:exp6}
	\end{minipage}
	\hfill
	\begin{minipage}[t]{0.49\linewidth}
		\includegraphics[width=40mm,height=30mm]{figure/exp-ucr.eps}
		\caption{Scalability}
		\label{fig:exp2}
\end{minipage}
\end{figure}


\begin{figure}[t]
	\centering
	\begin{tabular}[htbp]{cc}
		\includegraphics[width=40mm,height=30mm]{figure/dp-new-10.eps} &
		\includegraphics[width=40mm,height=30mm]{figure/dp-new-100.eps} \\
		\footnotesize (a) $\varepsilon = 10$ & \footnotesize (b) $\varepsilon = 100$ \\
	\end{tabular}
	\caption{\label{fig:exp7}Effect of dynamic window segmentation}
\end{figure}

It can be seen that KV-match${_{\text{DP}}}$ is faster than UCR Suite under both ED and DTW measures by almost two to three orders of magnitude. For trillion-length ($10^{12}$) series, we can process queries by 127s (under ED measure) and 243s (under DTW measure) on average, which shows great scalability.

\subsection{KV-match$_{\textit{DP}}$ vs. the Basic KV-match}
\label{sec:experiment_dp}
In this experiment, we compare the runtime between KV-match$_{\text{DP}}$ and KV-match for RSM queries.
We build 5 KV-indexes with $w$ as $25, 50, 100, 200, 400$ respectively.
For KV-match$_{\text{DP}}$, we set $\Sigma=\left\{25,50,100,200,400\right\}$ to use all these indexes.
%While KV-match is executed for each index respectively.
% only one index, and the window length of the indexes are $25, 50, 100, 200, 400$ respectively, and in KV-match$_{DP}$, $\Sigma=\left\{25,50,100,200,400\right\}$.
The experiment is conducted with local file version on length-$10^9$ real dataset. Because the performance of a single index is highly related to the length of queries, we test the runtime of variable query lengths. Fig.~\ref{fig:exp7} (a) and (b) show the results in the case of $\varepsilon=10$ (representing low selectivity) and $\varepsilon=100$ (representing high selectivity) respectively.

It can be seen that in most cases, KV-match$_{\text{DP}}$ outperforms all single indexes. On the contrary, the index with small window length is suitable only for shorter queries, while the index with large window length only works well on longer queries. The results verify the effectiveness of our query segmentation algorithm. KV-match$_{\text{DP}}$ can utilize the pruning power of multiple window lengths and leverage the data characteristics of the query sequences.



%\subsection{Window Reduction and Reordering}
%\label{sec:experiment_terminate}
%In this experiment, we verify the effectiveness of the window reduction and window reordering techniques. The experiments are conducted with local file version on length-$10^9$ real dataset for RSM queries under ED measure.
%
%The runtime of query processing with and without window reduction technique are shown in Figure~\ref{fig:exp5}.
%%We compare the runtime of query processing with and without window reduction technique. % Moreover, we test the accuracy of estimating time $T_2$. The accuracy is computed as $1-\frac{|\hat{N_r}-N_r|}{N_r}$, where $\hat{N_r}$ is the actual rounds executed in phase 1 with window reduction, and $N_r$ is the number of rounds in phase 1 which can achieve the smallest total time $T$.
%%The results are shown in Figure~\ref{fig:exp5}.
%It shows that window reduction technique improves the efficiency about 20\%, which verifies our learn-based approach in Section~\ref{sec:optimization_early}.
%
%%\begin{figure}[htbp]
%%	\centering
%%	\begin{tabular}[h]{cc}
%%		\includegraphics[width=40mm,height=30mm]{figure/exp5-test.eps} &
%%		\includegraphics[width=40mm,height=30mm]{figure/exp5-time.eps} \\
%%		(a) Accuracy & (b) Time \\
%%	\end{tabular}
%%	\caption{\label{fig:exp5}Effect of window reduction}
%%\end{figure}
%
%%Figure~\ref{fig:exp5}(a) shows that our estimation method achieves good accuracy. In most cases, the accuracy is higher than 98\%. As shown in Figure~\ref{fig:exp5}(b), window reduction improves the efficiency about 20\%.
%
%%\subsection{Effects of Optimizations}
%%In the experiments of this section, we  of the proposed optimization techniques in Section~\ref{sec:optimization}. The experiments are conducted with the same settings except the optimization being analyzed.
%
%
%%\needspace{5mm}
%%\subsection{Effect of Window Reordering}
%%\label{sec:experiment_order}
%
%
%The runtime of query processing with and without window reordering technique are shown in Figure~\ref{fig:exp3}.
%
%It shows that window reordering technique improves the efficiency greatly, especially in the case of high selectivities.
%
%\begin{figure}[t]
%	\begin{minipage}[t]{0.49\linewidth}
%		\includegraphics[width=40mm,height=30mm]{figure/exp5-time.eps}
%		\caption{Window reduction}
%		\label{fig:exp5}
%	\end{minipage}
%	\hfill
%	\begin{minipage}[t]{0.49\linewidth}
%		\includegraphics[width=40mm,height=30mm]{figure/exp3-1-time.eps}
%		\caption{Window reordering}
%		\label{fig:exp3}
%	\end{minipage}
%\end{figure}


%\needspace{1cm}


==> tex/index.tex <==
%\needspace{1cm}
\section{KV-\MakeLowercase{index}}
\label{sec:index}
In this section, we present our index structure KV-index, and the index building algorithm.

\subsection{Index Structure}
\label{sec:index_structure}
%In the index in Fig.~\ref{fig:example}, one entry corresponds to one sliding window of $X$. This index structure has approximately equal number of entries to $|X|$, and causes a huge space cost. To avoid it, we propose a more compact index structure which utilizes the data locality property of time series data, that means the values of adjacent time points may be close. In consequence, the mean values of adjacent sliding windows will be similar either.

The index structure in Fig.~\ref{fig:example} has approximately equal number of entries of $|X|$, which causes a huge space cost. To avoid that, we propose a more compact index structure which utilizes the data locality property, that is, the values of adjacent time points may be close. In consequence, the mean values of adjacent sliding windows will be similar too.

Logically, KV-index consists of ordered rows of key-value pairs. The key of the $i$-th row, denoted as $K_i$, is a \emph{range} of mean values of sliding windows, that is,
$K_i=[low_i, up_i)$,
where $low_i$ and $up_i$ are the left and right endpoint of the mean value range of $K_i$ respectively. It is a left-closed-right-open range, and the ranges of adjacent rows are disjoint.

The corresponding value, denoted as $V_i$, is the set of sliding windows whose mean values fall within $K_i$. To facilitate the expression, we represent each window by its position, that is, we represent sliding window $X(j, w)$ with $j$. To further save the space cost and also facilitate subsequence matching algorithm, we organize the window positions in $V_i$ as follows. The positions in $V_i$ are sorted in ascending order, and consecutive ones are merged into a \emph{window interval}, denoted as $\textit{WI}$. So $V_i$ consists of one or more sorted and non-overlapped window intervals.

\begin{definition}[Window Interval]
	We combine the $l^{th}$ to $r^{th}$ length-$w$ sliding windows of $X$ as a window interval $\textit{WI} = [l, r]$, which contains a set of sliding windows $\{X(l,w), X(l+1,w), \cdots, X(r,w)\}$, where $1 \leq l \leq r \leq |X|-w+1$.
\end{definition}

In the following descriptions, we use $j \in \textit{WI}$ to denote the window position $j$ belonging to the window interval $\textit{WI}=[l,r]$, that is, $j \in [l, r]$. Moreover, we use $\textit{WI}.l$, $\textit{WI}.r$ and $|\textit{WI}|=r-l+1$ to denote the left boundary, the right boundary and the size of interval $\textit{WI}$ respectively. The overall number of window intervals in $V_i$ is denoted as $n_I(V_i)$, and the number of window positions in $V_i$ as $n_P(V_i)$. Formally, we have
\begin{align}
\label{eq:niv}
n_I(V_i) ={}& \big|\{\textit{WI}~|\textit{WI}\in V_i\}\big| \\
\label{eq:nov}
n_P(V_i) ={}& \sum_{\textit{WI}\in V_i} \big|\textit{WI}\big|
\end{align}

Fig.~\ref{fig:index} shows KV-index for Fig.~\ref{fig:example}. The first row indicates that there exists three sliding windows, $X(1000, 50)$, $X(1001, 50)$ and $X(1002, 50)$, whose mean values fall within the range $[1.5, 2.0)$. In the second row, three windows are organized into two intervals $[49, 50]$ and $[500,500]$. Thus $n_I(V_2)=2$ and $n_P(V_2)=3$. Note that, $[500,500]$ is a special interval which only contains one single window position.

%\begin{table}[htbp]
%	\caption{Index Structure}
%	\centering
%	\begin{tabulary}{\columnwidth}{CC}
%		\hline
%		\textbf{Key} & \textbf{Value} \\
%		\hline
%		{[}1.5, 2.0)   & {[1000, 1002]}    \\
%		{[}2.0, 3.0)   & {[49, 50], [500, 500]} \\
%		{[}3.0, 4.0)   & {[100, 100], [550, 550]}    \\
%		\dots\dots & \dots\dots      \\
%		{[}6.0, 7.5)   & {[150, 150], [1100, 1100]}   \\
%		\hline
%	\end{tabulary}
%	\label{tab:index}
%\end{table}

To facilitate the query processing, KV-index also contains a meta table, in which each entry is a quadruple as
$ \left<K_i, pos_i, n_I(V_i), n_P(V_i)\right>$,
where $pos_i$ is the offset of $i$-th row in the index file. Due to its small size, we can load the meta table to memory before processing the query. With the meta table, we can quickly determine the offset and the length of a scan operation by the simple binary search.

Physically, KV-index can be implemented as a local file, an HDFS file or an HBase table, because of its simple format. In this work, we implement two versions, a local file version and an HBase table version (details are in Section~\ref{sec:experiment}). In general, if a file system or a database supports the ``scan'' operation with start-key and end-key parameters, it can support KV-index. Due to space limitation, we provide details about the index implementation in our longer paper~\cite{arxiv}.



\subsection{Index Building Algorithm}
\label{sec:index_building_algorithm}
We build the index with two steps. First, we build an index in which all rows use the equal-width range of the mean values. Second, because data distribution is not balanced among rows, we merge adjacent rows to optimize the index. We first introduce a basic in-memory algorithm, which works for moderate data size. Then we discuss how to extend it to very large data scale.

In the first step, we pre-define a parameter $d$, which represents the range width of the mean values. The range of each row will be $[k\cdot d, (k+1) \cdot  d)$, where $k \in \mathbb{Z}$. We read series $X$ sequentially. A circular array is used to maintain the length-$w$ sliding window $X(i,w)$, and its mean value $\mu^X_{i}$ are computed on the fly. Assume the mean value of $S_{i-1}$, $\mu^X_{i-1}$, is in range $K_j$, and the mean value of the current window $S_i$, $\mu^X_{i}$, is also in $K_j$, we modify the current $\textit{WI}$ by changing its right boundary from $i-1$ to $i$. Otherwise, a new interval, $\textit{WI}=[i,i]$, will be added into certain row according to $\mu_i^X$.

The equal-width range can cause the zigzag style of adjacent rows. For example, the $V_i=\{[5,5], [7,7]\}$ and $V_{i+1}=\{[6,6],[8,8]\}$. Apparently, a better way is to merge these two rows so that the corresponding value becomes $V_i=[5,8]$.

In the second step, we merge adjacent rows with a greedy algorithm. We check the rows beginning from $\langle K_1, V_1\rangle$ and $\langle K_2, V_2\rangle$. Let the current rows be $\langle K_i, V_i\rangle$ and $\langle K_{i+1}, V_{i+1}\rangle$. The merging condition is whether $\frac{n_I(V_{i} \cup V_{i+1})}{n_I(V_{i}) + n_I(V_{i+1})}$ is smaller than $\gamma$, a pre-defined parameter. The rationale is that we merge the rows in which a large number of intervals are neighboring. If rows $\langle K_i, V_i\rangle$ and $\langle K_{i+1}, V_{i+1}\rangle$ are merged, the new key is $[low_i, up_{i+1})$, and the new value is $V_{i} \cup V_{i+1}$. Moreover, all neighboring window intervals from $V_i$ and $V_{i+1}$ are merged to one interval.

%Note that the row merging will be executed recursively. It happens that multiple continuous rows ($\ge$2) are merged.

The merge operation is actually a union operation between two ordered interval sequences, which can be implemented efficiently similar to the merge-sort algorithm. Since each window interval will be examined exactly once, its time complexity is $O(n_I(V_{i})+n_I(V_{i+1}))$.

If the size of index exceeds memory capacity, we build the index as follows. In the first step, we divide time series into segments, and build the fixed-width range index for each segment in turn. After all segments are processed, we merge the rows of different segments. The second step visits index rows sequentially, which can be also divided into sub-tasks. Since each step can be divided into sub-tasks, the whole index building algorithm can be easily adapted to distributed environment, like MapReduce.

\textbf{Complexity analysis.} The process of building KV-index consists of two steps, generating rows with the fixed width, and merging them into varied-width ones. The first step scans all data in stream fashion, computes the mean value, and inserts $\left<\mu, offset\right>$ entry into hash table. Note that the mean value of $X(i,l)$ can be computed based on that of $X(i-1,l)$, whose cost is $O(1)$. So the cost of the first step is $O(n)$. In the second step, we detect adjacent rows and merge them if necessary. Since the intervals are ordered within each row, the merge operation is similar to the merge sort, whose cost is $n_I(V_i)+n_I(V_{i+1})$. Therefore, the whole cost is $\sum_{i=1}^{D-1} n_I(V_i)+n_I(V_{i+1})$ ($D$ is the number of rows in first step). Because $n_I(V_i)\leq n_P(V_i)$ and $\sum_{i=1}^{D} n_P(V_i) =n-w+1$, we can infer that its cost is $O(2n)$. In summary, the complexity of building index is $O(n)$.

All previous index-based approaches, like FRM and General Match, are based on R-tree, whose building cost is $O(n \cdot log_2(n))$~\cite{r-tree}. Moreover, they use DFT to transform each $w$-size window of $X$, whose cost is $w \cdot log_2(w)$. So the total transformation cost is $O(n \cdot w \cdot log_2(w))$. Therefore, building KV-index is more efficient.


==> tex/introduction1.tex <==
\section{Introduction}
\label{sec:introduction}
Time series data are pervasive across almost all human endeavors, including medicine, finance and science. In consequence, there is an enormous interest in querying and mining time series data.~\cite{fast_shapelets, matrix_profile}. %In recent years, the volume of time series data has exploded, due to the popularity of new applications, such as data center management and IoT.

Subsequence matching problem is a core subroutine for many time series mining algorithms.
%The subsequence search problem on time series data has extensive applications in medical diagnosis, speech processing, climate analysis, financial analysis, etc.
Specifically, given a long time series $X$, for any query series $Q$ and a distance threshold $\varepsilon$, the subsequence matching problem finds all subsequences from $X$, whose distance with $Q$ falls within the threshold $\varepsilon$. %However, although this problem has been extensively studied, there is still a gap between the existing processing techniques and the demanding performance of TSDB~\cite{kdd12,dsms} due to two challenges.

%First, in order to make meaningful comparisons between two time series, both query and the matched subsequences must be z-normalized first, which can eliminate the effect of offset shifting and amplitude scaling~\cite{kdd12}.

FRM~\cite{frm94} is the pioneer work of subsequence matching. Many approaches have been proposed, either to improve the efficiency~\cite{vldb12,gmatch02} or to deal with various distance functions~\cite{tods11,vldb07}, such as Euclidean distance and Dynamic Time Warping. However, \emph{all} these approaches only consider the raw subsequence matching problem (RSM for short).
In recent years, researchers realize the importance of the subsequence normalization~\cite{kdd12}. It is more meaningful to compare the z-normalized subsequences, instead of the raw ones. UCR Suite~\cite{kdd12} is the state-of-the-art approach to solve the normalized subsequence matching problem (NSM for short).
%That is, given one long time series $X$, for any query series $Q$ and a distance threshold $\varepsilon$, the NSM problem finds all subsequences from $X$, which satisfies $D(\hat{S},\hat{Q})\leq \varepsilon$.
%More recently, another approach~\cite{edbt17} was proposed to speed up the UCR Suite by designing a more powerful lower bound.

The NSM approach suffers from two drawbacks. First, it needs to scan the full time series $X$, which is prohibitively expensive for long time series. For example, for a time series of length $10^9$, UCR Suite needs more than 100 seconds to process a query of length 1,000. \cite{kdd12} analyzed the reason why it is impossible to build the index for the NSM problem. Second, the NSM query may output some results not satisfying users' intent. The reason is that NSM fully ignores the offset shifting and amplitude scaling. However, in real world applications, the extent of offset shifting and amplitude scaling may represent certain specific physical mechanism or state. Users often only hope to find subsequences within similar state as the query. We illustrate it with an example.

\linespread{0.98}

\begin{figure}
	\centering
	\footnotesize
	\begin{tabular}{@{}crr@{}}
		\multirow{8}{0.6\linewidth}{\includegraphics[width=1.1\linewidth]{figure/1-2-3-indoor-acceleration-x-exclude-14-15-20-21-2.eps}}~
		& & \\
		& \multicolumn{2}{c}{(c) Information of Q}\\[1mm]
		\cline{2-3}
		& Offset \scriptsize{[Label]} & Length \\
		\cline{2-3}
		& 877 \scriptsize{[$Q$]} & 17,124 \\
		\cline{2-3}
		& & \\
		& \multicolumn{2}{c}{(d) Results of NSM}\\[1mm]
		\cline{2-3}
		& Offset \scriptsize{[Label]} & Distance \\
		\cline{2-3}
		& 252,492 \scriptsize{[$S_6$]} & 117.78 \\
		(a) PAMAP time series & 97,458 \scriptsize{[$S_4$]} & 130.80 \\
		\multirow{6}{0.6\linewidth}{\includegraphics[width=1.1\linewidth]{figure/1-2-3-indoor-acceleration-x-exclude-14-15-20-21-align-2.eps}}~ & 34,562 \scriptsize{[$S_3$]} & 138.12 \\
		& 161,416 \scriptsize{[$S_5$]} & 149.37 \\
		& $\cdots$ & $\cdots$ \\
		& 134,456 \scriptsize{[$S_1$]} & 164.88 \\ % 12th
		& 296,063 \scriptsize{[$S_2$]} & 166.74 \\
		& $\cdots$ & $\cdots$ \\
		\cline{2-3}
		(b) Aligned normalized subsequences & \multicolumn{2}{l}{$\star~~ \varepsilon=200.0$} \\
	\end{tabular}
	\caption{\label{fig:cnsm2}Illustrative example of cNSM}
\end{figure}

\linespread{0.91}

\textbf{Example 1.} The time series in Fig.~\ref{fig:cnsm2}(a) comes from the Physical Activity Monitoring for Aging People (PAMAP) dataset~\cite{fast_shapelets} collected from z-accelerometer at hand position. The monitored person conducts various activities alternatively, like sitting, standing, running and so on. Each activity lasts for about 3 minutes, and the data collection frequency is 100Hz. We use one subsequence corresponding to lying activity as the query ($Q$ in Fig.~\ref{fig:cnsm2}(c)) to find other ``lying'' subsequences. We issue a NSM query with $Q$, and Fig.~\ref{fig:cnsm2}(d) lists the top results. Unfortunately, all top-4 results corresponds to other activities. $S_3$ and $S_5$ correspond to sitting activity, while $S_4$ and $S_6$ correspond to breaking activity. Although $S_1$ and $S_2$ are the desired results (correspond to lying activity), they are ranked out of top-20. We show the normalized $Q$, $S_1$ and $S_6$ in Fig.~\ref{fig:cnsm2}(b). It is difficult to distinguish them after normalization.

By observing Fig.~\ref{fig:cnsm2}(a), one can filter the undesired results easily by adding an additional constraint: the output subsequences should have similar mean value as $Q$. In fact, this new type of NSM query, \emph{NSM plus some constraints}, is useful in many applications. We list two of them as follows,
\begin{itemize}
\item{(Industry application)} In the wind power generation field, LIDAR system can provide preview information of wind disturbances~\cite{branlard2009wind}. Extreme Operating Gust (EOG) is a typical gust pattern which is a phenomenon of dramatic changes of wind speed in a short period. Fig.~\ref{fig:wind} shows a typical EOG pattern. This pattern is important because it may generate damage on the turbine. All EOG pattern occurrences have the similar shape, and their fluctuation degree falls within certain range, because the wind speed cannot be arbitrarily high.
    %Both too steep or too flat fluctuation cannot be a real EOG pattern.
    If we hope to find all EOG pattern occurrences in the historical data, we can use a typical EOG pattern as the query, plus the constraint on the range of the values.
\item{(IoT application)} When a container truck goes through a bridge, the strain meter planted in the bridge will demonstrate a specific fluctuation pattern. The value range in the pattern depends on the weight of the truck. If we have one occurrence of the pattern as a query, we can additionally set a mean value range as the constraint to search container trucks whose weight falls within a certain range.
\end{itemize}

Note that the above applications cannot be handled by RSM query, because the existing offset shifting and amplitude scaling forces us to set a very large distance threshold, which will cause many false positive results.

Furthermore, to verify the universality of this new query type, we investigate the motif pairs in some popular real-world time series benchmarks.
%\footnote{You can download the datasets from "\url{http://www.cs.ucr.edu/~eamonn/MatrixProfile.html}" and "\url{https://github.com/GrammarViz2/grammarviz2_src}".}.
Motif mining~\cite{matrix_profile} is an important time series mining task, which finds a pair (or set) of subsequences with minimal normalized distance. For a motif subsequence pair, say $X$ and $Y$, we show the relative mean value difference ($\Delta$Mean$=\frac{|\mu^X-\mu^{Y}|}{\max-\min}$) and the ratio of standard deviation ($\Delta$Std$=|\frac{\sigma^X}{\sigma^Y}|$) in Fig.~\ref{fig:motif}
%\footnote{$\mu$ and $\sigma$ are mean value and standard deviation of a subsequence. $\max$ and $\min$ are the maximum and minimum value of the dataset.}.
We can see that although these pairs are found without any constraint (like NSM query), both mean value and standard deviation of motif subsequences are very similar. So we can find these pairs by the cNSM query, a NSM query plus a small constraint.

\begin{figure}[t]
	\begin{minipage}[t]{0.55\linewidth}
		\centering
		\raisebox{0.2\height}{\includegraphics[width=0.9\linewidth]{figure/wind2.eps}}
		\caption{\label{fig:wind}EOG pattern}
	\end{minipage}%
	\hfill%
	\begin{minipage}[t]{0.44\linewidth}
		\centering
		\includegraphics[width=\linewidth]{figure/motif.eps}
		\caption{\label{fig:motif}Motif example}
	\end{minipage}%
\end{figure}

In this paper, we formally define a new subsequence matching problem, called \emph{constrained normalized subsequence matching problem} (cNSM for short). Two constraints, one for mean value and the other for standard deviation, are added to the traditional NSM problem. One exemplar cNSM query looks like ``given a query $Q$ with mean value $\mu^Q$ and standard deviation $\sigma^Q$, return subsequences $S$ which satisfy: (1) $Dist(\hat{S},\hat{Q})\leq 1.5$; (2) $|\mu^Q-\mu^S|\leq 5$; (3) $0.5\leq \sigma^Q/\sigma^S\leq 2$''. With the constraint, the cNSM problem provides a knob to flexibly control the degree of offset shifting (represented by mean value) and amplitude scaling (represented by standard deviation). Moreover, the cNSM problem offers us the opportunity to build index for the normalized subsequence matching.

\textbf{Challenges.} Solving the cNSM problem faces the following challenges. First, how can we process the cNSM query efficiently? A straightforward approach is to first apply UCR Suite to find unconstrained results, and then use mean value and standard deviation constraints to prune the unqualified ones. However, it still needs to scan the full series. Can we build an index and process the query more efficiently?

Second, users often conduct the similar subsequence search in an exploratory and interactive fashion. Users may try different distance functions, like Euclidean distance or Dynamic Time Warping. Meanwhile, users may try RSM and cNSM query simultaneously. Can we build a single index to support all these query types?

\textbf{Contributions.}
Besides proposing the cNSM problem, we also have the following contributions.
\begin{itemize}
\item We present the filtering conditions for four query types, RSM-ED, RSM-DTW, cNSM-ED and cNSM-DTW, and prove the correctness. The conditions enable us to build index and meanwhile guarantee no false dismissals.
\item We propose a new index structure, KV-index, and the query processing approach, KV-match, to support all these query types. The biggest advantage is that we can process various types of queries efficiently with a single index. Moreover, KV-match only needs a few numbers of \emph{sequential scans} of the index, instead of many random accesses of tree nodes in the traditional R-tree index, which makes it much more efficient.
\item Third, to support the query of arbitrary lengths efficiently, we extend KV-match to KV-match$_{\text{DP}}$, which utilizes multiple indexes with different window lengths. We conduct extensive experiments. The results verify the efficiency and effectiveness of our approach.
\end{itemize}


%First, we propose a novel definition of \emph{constrained normalized subsequence matching problem} (cNSM). Although the NSM problem can eliminate the effect of offset shifting and amplitude scaling, it may find unexpected matching subsequences, which is irrelevant to the query pattern in domain knowledge. In contrast, the proposed cNSM problem provides a knob to flexibly control the degree of offset shifting (represented by mean value) and amplitude scaling (represented by standard deviation). We illustrate it with the example in Figure~\ref{fig:cnsm}. Figure 1(a) shows an example query $Q$ and three subsequences $S_1$, $S_2$ and $S_3$. The detailed statistics are shown in Figure~\ref{fig:cnsm}(c). Figure~\ref{fig:cnsm}(b) shows the corresponding normalized series, denoted as $\hat{Q}$, $\hat{S}_1$, $\hat{S}_2$ and $\hat{S}_3$ respectively. It can be seen that all these four normalized sequences are similar. However, users may only want $S_3$ as the correct answer, since both mean value and standard deviation of $S_3$ are similar to those of $Q$. In contrast, $S_1$ has too much offset shifting (its mean value $0.10\gg -1.12$) and $S_2$ has too much amplitude shrinking (its standard deviation $0.06\ll 0.15$). As another real-world example of temperature monitoring, by setting proper offset shifting factor, cNSM can find specific fluctuation in winter and filter similar ones in summer.

The rest of the paper is organized as follows. We present the preliminary knowledge and problem statements in Section~\ref{sec:preliminary}. In Section~\ref{sec:motivation} we introduce the theoretical foundation and motivate the approach. Section~\ref{sec:index} and \ref{sec:matching} describe our index structure, index building algorithm and query processing algorithm. Section~\ref{sec:dynamic} extends our method to use multi-level indexes with different window lengths. %Our implementation details with TSDB are described in Section~\ref{sec:implementation}.
The experimental results are presented in Section~\ref{sec:experiment} and we discuss related works in Section~\ref{sec:related}. Finally, we conclude the paper and look into the future work in Section~\ref{sec:conclusion}.
%TODO: is there future work and implementation section?



==> tex/theoretical.tex <==
\needspace{10mm}
\section{Theoretical Foundation and \\Approach Motivation}
\label{sec:motivation}
In this section, we establish the theoretical foundation of our approach. We propose a condition to filter the unqualified subsequences. For all four types of queries, the conditions share the same format, which enables us to support all query types with a single index.

Specifically, for the query $Q$ and the subsequence $S$ of length-$m$, we segment them into aligned disjoint windows of the same length $w$. The $i$-th window of $Q$ (or $S$) is denoted as $Q_i$ (or $S_i$), ($1\leq i \leq p=\left\lfloor\frac{m}{w}\right\rfloor$), that is, $Q_i=(q_{(i-1)* w+1},\cdots,q_{i* w})$.

For each window, we hope to find one or more features, based on which we can construct the filtering condition. In this work, we choose to utilize one single feature, the mean value of the window. The advantages are two-folds. First, with a single feature, we can build a one-dimensional index, which improves the efficiency of index retrieval greatly. Second, the mean value allows us to design the condition for both RSM and cNSM query.

We denote mean values of $Q_i$ and $S_i$ as $\mu_i^Q$ and $\mu_i^S$. The condition consists of $p$ number of ranges. The $i^{th}$ one is denoted as $[\textit{LR}_i,\textit{UR}_i]$ ($1\leq i \leq p$). If $S$ is a qualified subsequence, for any $i$, $\mu_i^S$ must fall within $[\textit{LR}_i,\textit{UR}_i]$. If any $\mu_i^S$ is outside the range, we can filter $S$ safely.

%We fir present the condition for simplest case, RSM-ED query, illustrate the index and the matching algorithm. Then we extend it to other query types.

\subsection{RSM-ED Query Processing}
\label{section:RSM}
In this section, we first present the condition for the simplest case, RSM-ED query, and then illustrate our approach.

%We propose a condition to filter the unqualified subsequences. For all four types of queries, the conditions share the same format, which enables us to support all query types with a single index. Specifically, for any query $Q$ and subsequence $S$ of length-$m$, we segment them into aligned disjoint windows of same length $w$. The $i$-th window of $Q$ (or $S$) is denoted as $Q_i$ (or $S_i$), ($1\leq i \leq p=\left\lfloor\frac{m}{w}\right\rfloor$). Formally, $Q_i=(q_{(i-1)\cdot w+1},\cdots,q_{i\cdot w})$. The mean values of $S_i$ and $Q_i$ are $\mu_i^S$ and $\mu_i^Q$ respectively.

\begin{lemma}
	\label{lemma:RSM-ED}
	If $S$ and $Q$ are in $\varepsilon$-match under \textit{ED} measure, that is, $\textit{ED}(S,Q)\leq \varepsilon$, then $\mu_i^S~(1\leq i\leq p)$ must satisfy
	\begin{equation}
	\mu^{S}_{i} \in \left[\mu^{Q}_{i} - \frac{\varepsilon}{\sqrt{w}}, \mu^{Q}_{i} + \frac{\varepsilon}{\sqrt{w}}\right]
    \label{eq:RSM-ED}
	\end{equation}
	\proof
	Based on the ED definition, we have
	\begin{equation}
	\textit{ED}^2\left(S, Q\right) = \sum_{k=1}^{n}\left({s_k} - {q_k}\right)^{2} \geq
	\sum_{j=(i-1)* w +1}^{i* w}\left({s_j} - {q_j}\right)^{2} \nonumber
	\end{equation}
	where $1 \leq i \leq p$. According to the corollary in $\cite{vldb00}$,
	\begin{equation}
	\sum_{j=(i-1)* w +1}^{i* w}\left({s_j} - {q_j}\right)^{2} \geq
	{w} * \left(\mu^{S}_{i} - \mu^{Q}_{i}\right)^{2} \nonumber
	%\label{eq:origin}
	\end{equation}
	If $D\left(S, Q\right) \leq \varepsilon$, after inequality transformation, it should hold that $\left(\mu^{S}_{i} - \mu^{Q}_{i}\right)^{2} \leq \frac{\varepsilon^2}{w}$, so we get Eq.~(\ref{eq:RSM-ED}).
%	\begin{equation}
%	\mu^{S}_{i} \in \left[\mu^{Q}_{i} - \frac{\varepsilon}{\sqrt{w}}, \mu^{Q}_{i} + \frac{\varepsilon}{\sqrt{w}}\right] \nonumber
%	\end{equation}
%	where $1 \leq i \leq p$.
	\qed
\end{lemma}

\begin{figure}[t]
	\centering
	\includegraphics[width=\linewidth]{figure/example.eps}
	\caption{Illustrative example}
	\label{fig:example}
\end{figure}

Now we illustrate our approach with the example in Fig.~\ref{fig:example}. $X$ is a long time series, and $Q$ is the query sequence of length $161$. The goal is to find all length-$161$ subsequences $S$ from $X$, which satisfy $\textit{ED}(S,Q)\leq \varepsilon$. The parameter of the window length $w$ is set to 50. We split $Q$ into three disjoint windows of length $50$, $Q_1$, $Q_2$, $Q_3$\footnote{We can ignore the remain part $Q(151, 11)$ without sacrificing the correctness since Lemma~\ref{lemma:RSM-ED} is a \textit{necessary condition} for RSM.}. According to Lemma~\ref{lemma:RSM-ED}, for any qualified subsequence $S$, the mean value of the $i^{th}$ disjoint window $S_i$ must fall within the range $\left[\mu^{Q}_{i} - \frac{\varepsilon}{\sqrt{50}}, \mu^{Q}_{i} + \frac{\varepsilon}{\sqrt{50}}\right]$ ($i=1,2,3$). To facilitate finding the windows satisfying this condition, we build the index as follows. We compute the mean values of all sliding windows $X(j,w)$, denoted as $\mu(X(j,w))$, and build a sorted list of $\left<\mu(X(j,w)),j\right>$ entries. With this structure, we find the candidates in two steps. First, for each window $Q_i$, we obtain all sliding windows whose mean values fall within $\left[\mu^{Q}_{i} - \frac{\varepsilon}{\sqrt{50}}, \mu^{Q}_{i} + \frac{\varepsilon}{\sqrt{50}}\right]$ by a single \emph{sequential scan} operation. We denote the found windows for $Q_i$ as $\textit{CS}_i$. Then, we generate the final candidates by \emph{intersecting} windows in $\textit{CS}_1$, $\textit{CS}_2$ and $\textit{CS}_3$.

In Fig.~\ref{fig:example}, sliding windows in $\textit{CS}_1$, $\textit{CS}_2$ and $\textit{CS}_3$ are marked with ``triangle'', ``cross'' and ``circle'' respectively. The only candidate is $X(50,161)$, because  $X(50,50)\in \textit{CS}_1$, $X(100,50)\in \textit{CS}_2$ and $X(150,50)\in \textit{CS}_3$. %Our index is similar as the sorted list, but is more compact.

%The simplified index is shown in Figure~\ref{fig:example} (more details are discussed in Section~\ref{sec:index}). It is constructed based on all length-$w$ \textit{sliding windows} of $X$. %In this example, $w=50$.
%For each window $X(j,50)$ ($1\leq j\leq |X|-49$), index has an entry $\left<\mu(X(j,50)), j\right>$. All entries are sorted according to the mean values. For example, the first row $\left<1.7, 1000\right>$ indicates that the mean value of window $X(1000,50)$ is $1.7$.
%
%To process query $Q$, we segment $Q$ into three disjoint windows of length $50$, $Q(1,50)$, $Q(51,50)$, $Q(101,50)$, and compute the mean values $\mu^{Q}_{1}$, $\mu^{Q}_{2}$ and $\mu^{Q}_{3}$ respectively\footnote{We can ignore the remain part $Q(151, 11)$ without sacrificing the correctness since Lemma~\ref{lemma:RSM-ED} is a \textit{necessary condition} for RSM.}. Then we find potential candidates based on the index as follows. First, we ``scan'' the index with range $\left[\mu^{Q}_{1} - \frac{\varepsilon}{\sqrt{50}}, \mu^{Q}_{1} + \frac{\varepsilon}{\sqrt{50}}\right]$, and record the set of obtained windows as $CS_1$, marked with ``triangle'' in Figure~\ref{fig:example}.  Next, we find $CS_{2}$ and $CS_{3}$ by scanning the index with ranges $\left[\mu^{Q}_{2} - \frac{\varepsilon}{\sqrt{50}}, \mu^{Q}_{2} + \frac{\varepsilon}{\sqrt{50}}\right]$ and $\left[\mu^{Q}_{3} - \frac{\varepsilon}{\sqrt{50}}, \mu^{Q}_{3} + \frac{\varepsilon}{\sqrt{50}}\right]$, which are marked as ``cross'' and ``circle'' respectively. Then we generate the final candidate set from $CS_i$'s ($1\leq i\leq 3$) with an ``intersection" operation. The only candidate is $X(50,161)$, because  $X(50,50)\in CS_1$, $X(100,50)\in CS_2$ and $X(150,50)\in CS_3$. Finally, we fetch the candidate and compute the real distance.

%\begin{figure*}[t]
%	\begin{minipage}{0.7\linewidth}
%		\centering
%		\includegraphics[height=38mm]{figure/example.eps}
%		\caption{Illustrative example}
%		\label{fig:example}
%	\end{minipage}
%	\hfill
%	\begin{minipage}{0.3\linewidth}
%		\centering
%		\includegraphics[height=38mm]{figure/range.eps}
%		\caption{\label{fig:range}Legal range of $a$ and $b$}
%	\end{minipage}
%\end{figure*}

\subsection{Range for cNSM-ED Query}
\label{section:cNSM}
%Designing the range for the cNSM-ED query is more challenging, because we design the range on the raw data series while the distance is computed between the normalized subsequences. For the NSM query, the range does not exist at all. A simple example can illustrate it. Let $Q=(1,1,1,-1,-1,-1)$ and $S=(100,100,100,-100,-100,-100)$. Although the values of $S$ is much larger, it still holds that $\textit{ED}(\hat{Q},\hat{S})=0$. In fact, the values in $S$ can be arbitrarily large, which causes the mean value of a window can be arbitrarily large too.
%
%Fortunately, the constraints of mean value and standard deviation can avoid this extreme case and enable us to find a range for cNSM query. The rationale is as follows. If certain $\mu_i^S$ is a very large positive value, to make the global mean value fall within the constraint, there must exist another window $S_{j}$, whose $\mu_{j}^S$ is a negatively large value. However, these two large mean values, one positive and the other negative, will make the global standard deviation too large to fall outside the standard deviation constraint.

We solve the cNSM problem based on KV-index either. For the given query $Q$, we determine whether a subsequence $S$ is $(\varepsilon, \alpha, \beta)$-match with $Q$ by checking the raw subsequence $S$ directly. Specifically, we achieve this goal by designing the range $[LR_i, UR_i]$ for each query window $Q_i$. For any subsequence $S$, if any $\mu^S_i$ falls outside this range, $S$ cannot be $(\varepsilon, \alpha, \beta)$-match with $S$ and we can filter $S$ safely. We illustrate it with an example. Let $Q=(1,1,-1,-1)$, $w=2$, $(\alpha,\beta)=(2,1)$ and $\varepsilon=0$~\footnote{To make the example simple enough, we set $\varepsilon$ as 0.}. By simple calculation, we obtain $\mu^Q_1=1$ and $\sigma^Q=1.1547$. For any length-4 subsequence $S$, if only $\mu^S_1=4$, we can infer that $S$ cannot be matched with $Q$ without checking the whether $\hat{S}$ satisfies the cNSM condition, as follows. To make $ED(\hat{Q},\hat{S})=0$, $\mu^S_2$ must be -4. If it is the case, $\sigma^S$ is 4.6188 at least. However, $\frac{\sigma^S}{\sigma^Q}>2$, which violates the cNSM condition.

%Similarly, given query $Q$ and a subsequence $S$ of length-$m$, can we find a range for each $\mu_i^S$ ($1\leq i\leq p$), so that only if certain $\mu_i^S$ falls outside the corresponding range, $S$ and $Q$ cannot be in $(\varepsilon, \alpha, \beta)$-match under ED measure, and we can prune $S$ safely? The answer is yes.
%
%Next we present the range for cNSM-ED query. Let $\mu^{S}$ and $\mu^{Q}$ be the global mean values of $S$ and $Q$, $\sigma^{S}$ and $\sigma^{Q}$ be the standard deviations. $\hat{S}$ and $\hat{Q}$ are the normalized series of $S$ and $Q$, as Eq.~\ref{eq:normaliedseries}, respectively.

%We find Let $a=\frac{\sigma^{S}}{\sigma^{Q}}$ and $b=\mu^S-\mu^Q$.
%First, we find the range for any $(a,b)$ pair where $a\in [\frac{1}{\alpha}, \alpha]$ and $b \in [-\beta,\beta]$. Then we union all ranges for all possible $(a,b)$ to obtain the final range.

Now we formally give the range for cNSM-ED query. Let $\mu^{S}$ and $\mu^{Q}$ be the global mean values of $S$ and $Q$, $\sigma^{S}$ and $\sigma^{Q}$ be the standard deviations, $\hat{S}$ and $\hat{Q}$ be the normalized $S$ and $Q$ respectively.

%Lemma~\ref{lemma:cNSM-ED} and \ref{lemma:cNSM-DTW} give the condition for cNSM queries under ED and DTW measures respectively. It is worth noting that since the index is built upon the raw time series $X$, so the range for the normalized query is still established for the raw subsequences.

\begin{lemma}
\label{lemma:cNSM-ED}
	If $S$ and $Q$ are in $(\varepsilon, \alpha, \beta)$-match under \textit{ED} measure, that is, $\textit{ED}(\hat{S},\hat{Q})\leq \varepsilon$, then $\mu^S_i~(1\leq i\leq p)$ satisfies
%	\begin{flalign*}
%	&& \mu_i^S &\in \left[v_{min}+\mu^Q-\beta, v_{max}+\mu^Q+\beta\right] & \tag{\the\numexpr\value{equation}+1\relax}\\
%	where && v_{min} &= \mathop {\min} \limits_{t \in \{\alpha, \frac{1}{\alpha}\}} \left\{t \cdot \left(\mu_i^Q-\mu^Q- \frac{\varepsilon  \sigma^Q}{\sqrt{w}}\right) \right\}, &\\
%	and   && v_{max} &= \mathop {\max} \limits_{t \in \{\alpha, \frac{1}{\alpha}\}} \left\{t \cdot \left(\mu_i^Q-\mu^Q+ \frac{\varepsilon  \sigma^Q}{\sqrt{w}}\right) \right\}. &
%	\setcounter{equation}{\value{equation}+1}
%	\end{flalign*}
\begin{equation}
\mu_i^S \in \left[v_{\min}+\mu^Q-\beta, v_{\max}+\mu^Q+\beta\right]
\label{eq:lemma3}
\end{equation}
where\\
$v_{\min}= \tiny{~} \min \left(\alpha\cdot(\mu_i^Q-\mu^Q- \frac{\varepsilon  \sigma^Q}{\sqrt{w}}), \frac{1}{\alpha}\cdot(\mu_i^Q-\mu^Q- \frac{\varepsilon  \sigma^Q}{\sqrt{w}}) \right)$,\\
$v_{\max}= \max \left(\alpha\cdot(\mu_i^Q-\mu^Q+ \frac{\varepsilon  \sigma^Q}{\sqrt{w}}), \frac{1}{\alpha}\cdot(\mu_i^Q-\mu^Q+ \frac{\varepsilon  \sigma^Q}{\sqrt{w}}) \right)$.

	\proof
	Based on the normalized ED definition, we have
	%Let $D\big(\hat{S}, \hat{Q}\big)$ be the ED between normalized time series $\hat{S}$ and $\hat{Q}$,
	\small
	\begin{equation}
	\textit{ED}\big(\hat{S}, \hat{Q}\big) = \sqrt{\sum_{j=1}^{m}\left({\frac{s_j-\mu^S}{\sigma^S}} - {\frac{q_j-\mu^Q}{\sigma^Q}}\right)^{2}} \nonumber
	\end{equation}
	\normalsize
	
	Let $a=\frac{\sigma^{S}}{\sigma^{Q}}$ and $b=\mu^S-\mu^Q$, where $a \in [\frac{1}{\alpha}, \alpha]$ and $b \in [-\beta,\beta]$. If $\textit{ED}\big(\hat{S}, \hat{Q}\big) \leq \varepsilon$, it holds that
	\small
	\begin{equation}
	\sum_{j=1}^{m}\left({\frac{s_j-\mu^Q-b}{a \sigma^Q}} - {\frac{q_j-\mu^Q}{\sigma^Q}}\right)^{2} \leq \varepsilon^2  \nonumber
	\end{equation}
	\normalsize
	%We denote $\mu_i^S(x,y)$ as a function of the mean value of the $i$-th window of $S$ $(1\leq i\leq q)$ under $\frac{\sigma^{S}}{\sigma^{Q}} = x$ and $\mu^S-\mu^Q = y$ $(x \in [\frac{1}{\alpha}, \alpha]$, $y \in [-\beta,\beta])$.
	
	According to the corollary in $\cite{vldb00}$, similar to Lemma~\ref{lemma:RSM-ED}, for the $i$-th window $S_i$ and $Q_i$, we have
	\small
	\begin{equation}
	\left({\frac{\mu_i^S-\mu^Q-b}{a \sigma^Q}} - {\frac{\mu_i^Q-\mu^Q}{\sigma^Q}}\right)^{2} \leq \frac{\varepsilon^2}{w}  \nonumber
	\end{equation}
	\normalsize
	
    By simple transformation, for any specific pair of $(a,b)$, we can get a range of $\mu_i^S$ as follows,
%	\begin{flalign}
%	\text{ } && \mu_i^S \in  \bigg[&\left(\mu_i^Q-\mu^Q-\frac{\varepsilon  \sigma^Q}{\sqrt{w}}\right) a + b + \mu^Q, &\label{eq:rRSM-ED}\\
%	&&                    & \left(\mu_i^Q-\mu^Q+\frac{\varepsilon  \sigma^Q}{\sqrt{w}}\right) a + b + \mu^Q\bigg] & \nonumber
%	\end{flalign}
	\small
	\begin{equation}
	\mu_i^S \in  \bigg[\left(\mu_i^Q-\mu^Q-\frac{\varepsilon  \sigma^Q}{\sqrt{w}}\right) a + b + \mu^Q,  \left(\mu_i^Q-\mu^Q+\frac{\varepsilon  \sigma^Q}{\sqrt{w}}\right) a + b + \mu^Q\bigg] \nonumber
	%\label{eq:rRSM-ED}
	\end{equation}
	\normalsize
	
%Next, we prove the range in Eq.~\ref{eq:lemma3} is the union of ranges for all pairs $(a,b)$ satisfying $a \in [\frac{1}{\alpha},\alpha]$ and $b \in [-\beta,\beta]$.
For ease of description, we assign $\mu_i^Q-\mu^Q-\frac{\varepsilon \sigma^Q}{\sqrt{w}}=A$ and $\mu_i^Q-\mu^Q+\frac{\varepsilon \sigma^Q}{\sqrt{w}}=B$.
	
	The final range $[\textit{LR}_i, \textit{UR}_i]$ should be
	\begin{flalign*}
	\Bigg[\min\limits_{
		\substack{a \in [\frac{1}{\alpha},\alpha]\\
			b \in [-\beta,\beta]}}
	\left\{A  a + b + \mu^Q\right\},
	\max\limits_{
		\substack{a \in [\frac{1}{\alpha},\alpha]\\
			b \in [-\beta,\beta]}}
	\left\{B  a + b + \mu^Q\right\}
	\Bigg]
	\end{flalign*}
	
	As illustrated in Fig.~\ref{fig:range}, the rectangle represents the whole legal range of $a$ and $b$. Let $f(a,b)=A a+b+\mu^Q$ and $g(a,b)=B a+b+\mu^Q$. Apparently, both $f(a,b)$ and $g(a,b)$ increase monotonically for $b \in [-\beta,\beta]$. As for $a$, we have two cases,
	\begin{itemize}
		\item If $A \ge 0$, $f(a,b)$ increases monotonically for $a \in [\frac{1}{\alpha},{\alpha}]$. $f(a,b)$ is minimal when $a={\frac{1}{\alpha}}$ and $b={-\beta}$, which is represented by the point $p_3$ in Fig.~\ref{fig:range};
		\item If $A<0$, $f(a,b)$ decreases monotonically for $a \in [\frac{1}{\alpha},{\alpha}]$. $f(a,b)$ is minimal when $a={\alpha}$ and $b={-\beta}$, which is represented by the point $p_4$ in Fig.~\ref{fig:range}.
	\end{itemize}
	\begin{flalign*}
	\text{So} && \textit{LR}_i=\min\limits_{a \in [\frac{1}{\alpha},\alpha],
		b \in [-\beta,\beta]} f(a,b) &= \min\limits_{a \in \left\{\frac{1}{\alpha},\alpha \right\}} f(a,-\beta) &
	\end{flalign*}

    Note that formula $a \in \left\{\frac{1}{\alpha},\alpha\right\}$ means $a$ is either $\frac{1}{\alpha}$ or $\alpha$.
	
	Similarly, we can infer the maximal value of $g(a,b)$ as following two cases,
	\begin{itemize}
		\item If $B \ge 0$, $g(a,b)$ is maximal when $a={\alpha}$ and $b={\beta}$, which is represented by the point $p_2$ in Fig.~\ref{fig:range}.
		\item If $B<0$, $g(a,b)$ is maximal when $a={\frac{1}{\alpha}}$ and $b={\beta}$, which is represented by the point $p_1$ in Fig.~\ref{fig:range}.
	\end{itemize}
	\begin{flalign*}
	\text{So} && \textit{UR}_i=\max\limits_{a \in [\frac{1}{\alpha},\alpha],
		b \in [-\beta,\beta]} g(a,b) &= \max\limits_{a \in \left\{\frac{1}{\alpha},\alpha \right\}} g(a,\beta) &
	\end{flalign*}
	\qed
%	In summary, we can obtain
%	\begin{equation}
%	\mu_i^S \in \left[\min\limits_{a \in \left\{\frac{1}{\alpha}, \alpha \right\}}f(a,-\beta), \max\limits_{a \in \left\{\frac{1}{\alpha}, \alpha \right\}}g(a,\beta)\right] \nonumber
%	\end{equation}
%	which is equivalent to Eq.~\ref{eq:lemma3}.
\end{lemma}

\begin{figure}[t]
	\begin{minipage}[t]{0.4\linewidth}
		\centering
		\includegraphics[width=0.93\linewidth]{figure/range.eps}
		\caption{\label{fig:range}Legal Range of $(a,b)$}
	\end{minipage}%
	\hfill%
	\begin{minipage}[t]{0.58\linewidth}
		\centering
		\includegraphics[width=0.9\linewidth]{figure/index.eps}
		\caption{\label{fig:index}Index Structure}
	\end{minipage}%
\end{figure}

\vspace{-7mm}
\subsection{Range for RSM-DTW and cNSM-DTW Query}
Before introducing the ranges, we first review the query envelop and the lower bound of DTW distance, LB\_PAA~\cite{lb_paa}. To deal with DTW$_{\rho}$ measure, given length-$m$ query $Q$, the query envelop consists of two length-$m$ series, $L$ and $U$, as the lower and upper envelop respectively. The $i$-th elements of $L$ and $U$, denoted as $l_i$ and $u_i$, are defined as
\begin{center}
	$\displaystyle l_i=\min_{-\rho\leq r\leq \rho} q_{i+r}$ , $\displaystyle u_i=\max_{-\rho\leq r\leq \rho} q_{i+r}$.
\end{center}

LB\_PAA is defined based on the query envelop. $L$ and $U$ are split into $p$ number of length-$w$ disjoint windows, $(L_1,L_2,\cdots,L_p)$ and $(U_1,U_2,\cdots,U_p)$, in which $L_i=(l_{(i-1)\cdot w+1},\cdots,l_{i\cdot w})$ and $U_i=(u_{(i-1)\cdot w+1},\cdots,u_{i\cdot w})$ ($1\leq i \leq p=\lfloor \frac{m}{w}\rfloor$). The mean values of $L_i$ and $U_i$ are denoted as $\mu_i^L$ and $\mu_i^U$ respectively. For any length-$m$ subsequence $S$, the LB\_PAA is as follows,

\vspace{-4mm}
\small
\begin{equation}
\textit{LB\_PAA}(S,Q)=
\sqrt{\sum_{i=1}^{p}w\cdot
	\begin{lcases}
	&(\mu_i^S-\mu_i^U)^2 && \text{if~} \mu_i^S > \mu_i^U \\
	&(\mu_i^S-\mu_i^L)^2 && \text{if~} \mu_i^S < \mu_i^L \\
	&0 && \text{Otherwise} \\
	\end{lcases}
}
%~\leq \varepsilon
\label{eq:lb_paa}
\end{equation}
\normalsize
which satisfies $\textit{LB\_PAA}(S,Q)\leq \textit{DTW}_{\rho}(S,Q)$~\cite{lb_paa}.

%where $\mu_i^U$ and $\mu_i^L$ are the mean value of the $i$-th window of query envelop $U$ and $L$ respectively. Formally, the $i$-th window of $U$ (or $L$) is denoted as $U_i$ (or $L_i$), so $U_i=(u_{(i-1)\cdot w+1},\cdots,u_{i\cdot w})$, $L_i=(l_{(i-1)\cdot w+1},\cdots,l_{i\cdot w})$, where $1\leq i \leq p$.







%According to LB\_PAA~\cite{lb_paa} for DTW$_\rho$, if $D(S,Q) \leq \varepsilon$, we have

Now we give the ranges for RSM and cNSM under the DTW$_\rho$ measure in turn.
\begin{lemma}
	\label{lemma:RSM-DTW}
	If $S$ and $Q$ are in $\varepsilon$-match under \textit{DTW}$_\rho$ measure, that is, $\textit{DTW}_\rho (S,Q)\leq \varepsilon$, then $\mu_i^S~(1\leq i\leq p)$ satisfies
	\begin{equation}
	\mu^{S}_{i} \in \left[\mu^{L}_{i} - \frac{\varepsilon}{\sqrt{w}}, \mu^{U}_{i} + \frac{\varepsilon}{\sqrt{w}}\right]
    \label{eq:RSM-DTW}
	\end{equation}
	%\proof See Appendix~\ref{app:1}.
\end{lemma}



%\subsection{Condition for cNSM Problem}
%\label{section:cNSM}
%Let $\mu^{S}$ and $\mu^{Q}$ be the global mean values of $S$ and $Q$, $\sigma^{S}$ and $\sigma^{Q}$ be the standard deviations. $\hat{S}$ and $\hat{Q}$ are the normalized series of $S$ and $Q$, as Eq.~\ref{eq:normaliedseries}, respectively.
%%After normalization, we have $$\hat\mu_i^S=\frac{\mu_i^S-\mu^S}{\sigma^S},~ \hat\mu_i^L=\frac{\mu_i^L-\mu^Q}{\sigma^Q},~ \hat\mu_i^U=\frac{\mu_i^U-\mu^Q}{\sigma^Q}$$
%Lemma~\ref{lemma:cNSM-ED} and \ref{lemma:cNSM-DTW} give the condition for cNSM queries under ED and DTW measures respectively. It is worth noting that since the index is built upon the raw time series $X$, so the range for the normalized query is still established for the raw subsequences.



%Now we give the condition for cNSM under DTW$_\rho$ measure.
\begin{lemma}
	If $S$ and $Q$ are in $(\varepsilon, \alpha, \beta)$-match under \textit{DTW}$_\rho$ measure, that is, $\textit{DTW}_\rho(\hat{S},\hat{Q})\leq \varepsilon$, then $\mu^S_i~(1\leq i\leq p)$ satisfies
%	\begin{flalign*}
%	&& \mu_i^S &\in \left[v_{min}+\mu^Q-\beta, v_{max}+\mu^Q+\beta\right] & \tag{\the\numexpr\value{equation}+1\relax}\\
%	where && v_{min} &= \mathop {\min} \limits_{t \in \{\alpha, \frac{1}{\alpha}\}} \left\{t \cdot \left(\mu_i^L-\mu^Q- \frac{\varepsilon  \sigma^Q}{\sqrt{w}}\right) \right\}, &\\
%	and   && v_{max} &= \mathop {\max} \limits_{t \in \{\alpha, \frac{1}{\alpha}\}} \left\{t \cdot \left(\mu_i^U-\mu^Q+ \frac{\varepsilon  \sigma^Q}{\sqrt{w}}\right) \right\}. &
%	\setcounter{equation}{\value{equation}+1}
%	\end{flalign*}
	\label{lemma:cNSM-DTW}
	\begin{equation}
	\mu_i^S \in \left[v_{\min}+\mu^Q-\beta, v_{\max}+\mu^Q+\beta\right]
    \label{eq:lemma4}
	\end{equation}
	where\\
	$v_{\min}=\tiny{~} \min \left(\alpha\cdot(\mu_i^L-\mu^Q- \frac{\varepsilon  \sigma^Q}{\sqrt{w}}), \frac{1}{\alpha}\cdot(\mu_i^L-\mu^Q- \frac{\varepsilon  \sigma^Q}{\sqrt{w}}) \right)$,\\
	$v_{\max}= \max \left(\alpha\cdot(\mu_i^U-\mu^Q+ \frac{\varepsilon  \sigma^Q}{\sqrt{w}}), \frac{1}{\alpha}\cdot(\mu_i^U-\mu^Q+ \frac{\varepsilon  \sigma^Q}{\sqrt{w}}) \right)$.
	%\proof See Appendix~\ref{app:2}.
\end{lemma}

Due to the space limit, we omit the proof. Interested readers can find it in the long version paper~\cite{arxiv}.

%\subsection{Illustrative Example}
%\label{sec:example}


%Any subsequence of $X$, $S=X(j,161)$, also includes three disjoint windows, $S_1=X(j, 50)$, $S_2=X(j+50,50)$ and $S_3=X(j+100,50)$ where $1\leq j\leq |X|-160$. The corresponding mean values of these windows are $\mu^S_1$, $\mu^S_2$ and $\mu^S_3$. According to Lemma~\ref{lemma:RSM-ED}, if subsequence $S$ satisfies $ED\big(S,Q\big) \leq \varepsilon$, the mean values must satisfy the following formula simultaneously:
%\begin{equation}
%\label{eq:i}
%\mu^S_{i} \in{} \left[\mu^{Q}_{i} - \frac{\varepsilon}{\sqrt{50}}, \mu^{Q}_{i} + \frac{\varepsilon}{\sqrt{50}}\right]
%\end{equation}
%where $i\in \{1,2,3\}$. If for any $i$, Eq.~\ref{eq:i} is not satisfied, the subsequence $S$ can't be in $\varepsilon$-match with $Q$.%, and will not be the candidate.

%Our approach consists of two phases. In the first phase, we find candidate subsequences based on Eq.~\ref{eq:i}, \ref{eq:i50} and \ref{eq:i100}. In the second phase, we verify these candidates by calculating their real distance from $Q$. The key problem is how to find the candidates efficiently.


%It contains $|X|-w+1$ number of rows, each of which corresponds to a sliding window of $X$ with length $50$. Each row is a key-value pair. The key is a mean value of certain sliding window in $X$, and the value is the beginning point of this window. For example, the first row $\left<1.7, 1000\right>$ represents that the mean value of window $X(1000,50)$ is $1.7$. All rows in the index are ordered by the key in ascending order.

%After that, we fetch all candidate subsequences to verify them by calculating the true distance.
%The rationale is if subsequence $X(i,161)$ is a candidate, it holds that: 1) $X(i,50)\in CS_1$; 2) $X(i+50,50)\in CS_2$; 3) $X(i+100,50)\in CS_3$. We implement it efficiently.

%In the index of Figure~\ref{fig:example}, we mark $CS_1$ with ``triangle'', $CS_2$ with ``cross'' and $CS_3$ with ``circle''. The only candidate which satisfies all three equations is $X(50,161)$. For subsequence $X(500,161)$, although the first two windows, $X(500,50)$ and $X(550,50)$, satisfy Eq.~\ref{eq:i} and \ref{eq:i50}, the third window $X(600,50)$ is not contained by $CS_3$, so $X(500,161)$ will be pruned.

\textbf{Analysis}. We provide the ranges of mean value for all four query types, which means that we can support all queries with a single index. When processing different query types, the only difference is to use different ranges of $\mu_{i}^S$. This property is beneficial for exploratory search tasks.

%However, some issues need to be addressed. First, the index has almost the same size as the data, which is prohibitively large. We need to design a more compact index structure. Second, to support both long and short queries, using only one single index of fixed-length windows may suffer from sub-optimal efficiency. In next sections, we present our approach to address these issues.



